Hyperbolicity of varieties of log general type

These notes provide an overview of various notions of hyperbolicity for varieties of log general type from the viewpoint of both arithmetic and birational geometry. The main results are based on our paper entitled "Hyperbolicity and uniformity of varieties of log general type." They are expanded notes from a minicourse the authors gave as part of the Geometry and arithmetic of orbifolds workshop at UQ\'AM.

==> ff.tex <==
\section{Function Fields}\label{sec:ff}

Function fields in one variable and number fields share several properties. This deep analogy was observed in the second half of the 19th century; one of the first systematic treatments can be found in the famous paper by Dedekind and Weber \cite{Dedekind}. Further descriptions, due to Kronecker, Weil and van der Waerden, settled this profound connection which finally became formally completed with the scheme theory developed by Grothendieck.  

%In this chapter we are going to discuss how this analogy can be carried over Diophantine problems. In the first section we describe the analogous of Mordell Conjecture over function fields, which later became Manin's (although with a gap) and, independently, Grauert's Theorem in \cite{Manin1963} and \cite{Grauert1965} respectively. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Geometric Mordell}\label{sec:geo_mordell}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% As an example, one can ask whether the same result as Theorem \ref{thm:faltings} holds for function fields. In \cite{Lang_int} Serge Lang stated the following conjecture, which has become known as Geometric Mordell Conjecture over $\C$:

% \begin{conjecture}[Geometric Mordell]\label{conj:GeoMordell}
% Let $\calC$ be a curve of genus greater than 1 defined over a (complex) function field $F$ of an algebraic regular curve $\calB$, viewed as fibered surface $\pi: \calC \to \calB$. If the generic fiber $\calC_t$ has infinitely many $F$-rational points then there exists a covering $\calB' \to \calB$ such that the base change $\calC \times_{F} F'$, where $F'$ is the function field of $\calB'$, is isomorphic over $F'$ to $\calC_0 \times_\C F'$ for a curve $\calC_0$ defined over $\C$.
% \end{conjecture}

% One can immediately notice that the conclusion is not the same as in the number field case. This is because a bare translation could not work given the presence of isotrivial curves.

%as we are going to see in subsection\ref{subsec:mordell_ff} and the isotriviality question should be addressed. In order to properly describe the features of the previous Conjecture as well as the ideas behind its proof by Grauert \cite{Grauert1965} we need first a precise extension of arithmetic notions over number fields into the framework of function field arithmetic.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Function fields and Number fields}\label{subsec:ff_nf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As pointed out in the preface to this chapter function fields in one variable behave very similarly to number fields. We start this analogy with the following

\begin{definition}[Function Field]\label{def:FunctField}
A \emph{function field} $F$ over an algebraically closed field $k$ is a finitely generated field extension of finite transcendence degree over $k$. A function field \emph{in one variable}, or equivalently a function field of an algebraic curve, is a function field with transcendence degree equal to one
%, i.e. a field $F/k$ for which it exists an element $x$, transcendental over $k$, such that $K$ is a finite extension of $k(x)$.
\end{definition}

\begin{remark}
With the language of schemes the function field of a curve $X$, or more general of every integral scheme over an algebraic closed field, can be recovered from the structure sheaf $\calO_X$ in the following way: given any affine open subset of $X$, the function field of $X$ is the fraction field of $\calO_X(V)$. Moreover, if $\eta$ is the (unique) generic point of $X$, then the function field of $X$ is also isomorphic to the stalk $\calO_{X,\eta}$.
\end{remark}

The analogy between number fields and function fields of curves, also known as algebraic function fields in one variable, comes from the fact that one-dimensional affine integral regular schemes are either smooth affine curves over a field $k$ or an open subset of the spectrum of the ring of integers of a number field. Formally, given a number field $k$ with ring of integers $\calO_k$ the scheme $\Spec\calO_k$ is one dimensional affine and integral. From this analogy, several classical properties of number fields find an analogue in the theory of function field. In particular the theory of  heights can be defined over function fields.

\begin{definition}\label{def:FFabs}
Given a function field $F$ in one variable of a non singular curve $\calC$, each (geometric) point $P \in \calC$ determines a non trivial absolute value by
\[
\lvert f \rvert_{P}:= e^{-\ord_P(f)}.
\]
Moreover if $Q \neq P$ then the absolute values $\lvert \cdot \rvert_{Q}$ and $\lvert \cdot \rvert_{P}$ are not equivalent.
\end{definition}

\begin{remark}\leavevmode
\begin{itemize}
\item The definition could have been given more generally for function fields of algebraic varieties regular in codimension one (or rather for regular models of higher dimensional function fields), replacing the point $P$ with prime divisors. Extensions exist also for function fields over non-algebraically closed fields in which one should replace points with orbits under the absolute Galois group.
\item From the fact that any rational function $f$ on a projective curve has an associated divisor of degree zero, it follows that the set of absolute values satisfy the product formula.
\end{itemize}
\end{remark}

Given the set of absolute values $M_F$ for a function field in one variable $F$, normalized in such a way that they satisfy the product formula, heights can be defined for $F$ in the following way:

\begin{definition}\label{def:heightFF}
Let $F=k(\calC)$ be as before. For any $f \in F$ the \emph{height} of $f$ is
\[
h(f) = - \sum_{P \in \calC} \min \{ 0, \ord_P(f)\} = \sum_{P \in \calC} \max \{ 0, \ord_P(f)\}.
\]
In the same way for a point $g \in \PP^n(F)$, $g = (f_0 : \dots : f_n)$, its height is defined as
\[
h(g) = - \sum_{P \in \calC} \min_i \{ \ord_P(f_i) \}.
\]
\end{definition}

From the definition it follows that a rational function on a regular curve has no poles if and only if its height is zero if and only if it is constant on the curve.

We end this subsection with Table \ref{tab:NFFF}, which illustrates the interplay and the similarity between number fields and function fields. We stress in particular how each geometric object in the right column, in particular dominant maps and pullbacks, are analogous to purely arithmetic notions like extensions of fields and extensions of ideals. This analogy can be further explored using Arakelov Theory and extending the notion of divisors to number fields by suitably compactifying the affine curve $\Spec \calO_{k,S}$; in this framework an intersection theory can be defined for such compactified divisors sharing many analogous properties of intersection theory on the geometric side. We refer to \cite{Lang1988} for further details on this subject. 

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline 
Number Field & Function Field \\ 
\hline 
$\Z$ & $k [ x ]$	 \\
\hline 
$\Q$ & $k (x)$ \\ 
\hline 
$\Q_p$ & $k((x))$ \\ 
\hline 
$k$ finite extension of $\Q$ & $F$ function field of $\calC$ \\ 
\hline 
place & geometric point \\ 
\hline 
finite set of places & finite set of points \\ 
\hline 
ring of $S$-integers & ring of regular functions\\ 
\hline 
$\Spec \calO_{k,S}$ & Affine curve $\calC \setminus S$  \\ 
\hline 
product formula & $\deg$ principal divisor = 0 \\ 
\hline 
extension of number fields & dominant maps \\ 
\hline 
extension of ideals & pullback of divisors \\
\hline 
\end{tabular}
\caption{Number Fields and Function Fields analogy}\label{tab:NFFF} 
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mordell Conjecture for function fields}\label{subsec:mordell_ff}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Over function fields one cannot expect Faltings' Theorem \ref{thm:faltings} to hold as shown by the following examples.

\begin{example}
Let $\calC$ be a curve with $g(\calC) > 1$  defined over $\C$ and consider the trivial family $\calC \times \PP^1 \to \PP^1$. The family can be viewed as the curve $\calC$ (trivially) defined over the function field $\C( t)$ of $\PP^1$. All fibers of the family, being isomorphic to $\calC$ have genus greater than one. The Mordell Conjecture over function fields, without any other restriction, should imply that the set of $\C( t )$-rational points of $\calC$, i.e. there are finitely many sections $\PP^1 \to \calC \times \PP^1$. However this is easily seen to be false by considering constant sections $\PP^1 \to \{ P \} \times \PP^1$ for each point $P \in \calC(\C)$. In particular, the general type curve $\calC$ defined over $\C( t )$ has infinitely many $\C( t )$-rational points.
\end{example}

From the previous example one could guess that the problem relied on the fact that the family was a product and the curve $\calC$ was actually defined over the base field $\C$ rather than on the function field $\C ( t )$, i.e. the family was trivial. However, as the following example shows, things can go wrong even for non-trivial families.

\begin{example}[Gasbarri \cite{Gasbarrinotes}]
Consider the curve $\calC := (x + t y)^4 + y^4 -1$ defined over $\C( t )$. It has an associated fibration $\calC \to \PP^1$ whose generic fiber $\calC_{t_0} = (x + t_0 y)^4 + y^4 -1$ is a smooth projective curve of genus $g(\calC_{t_0}) = 3$. Again if we consider the same statement of Theorem \ref{thm:faltings} only replacing the number field with the function field $\C( t )$ we would expect that the number of $\C( t )$-rational points of $\calC$ to be finite. However we claim that $\calC(\C( t ))$ is infinite; to see this consider the equation $\alpha^4 + \beta^4 = 1$ over $\C^2$: it has infinitely many solutions. Each solution gives a $\C$-point of $\calC_{t_0}$, namely $(\alpha - t_0 \beta, \beta)$ proving the claim. Moreover the family is not trivial in the sense of the previous example, i.e. $\calC$ is not defined over $\C$. Notice however that each fiber of the family is isomorphic to the curve $x^4 + y^4 = 1$ via $x+t y \mapsto x$ and $y \mapsto y$.
\end{example}

Motivated by the previous examples we give the following:

\begin{definition}\label{def:isotrivial}
Given a family of irreducible, smooth projective curves $\calC \to \calB$ over a smooth base $\calB$, we say that the family is \emph{isotrivial} if $\calC_b$ is isomorphic to a fixed curve $\calC_0$ for $b$ in an open dense subset of $\calB$. With abuse of notation, we will say that a curve $\calC$ defined over a function field $F$ is \emph{isotrivial} if the corresponding fibration $\calC \to \calB$ is isotrivial, where $\calB$ is a curve with function field $F$.
\end{definition}

Isotriviality extends the notion of (birational) triviality for family of curves, i.e. a product of curves fibered over one of the factors is immediately isotrivial. At the same time this notion encompasses many other families that are not products, like the one defined in the previous example. However, after a cover of the base of the family, each isotrivial family becomes trivial; in particular the following easy lemma holds:

\begin{lemma}\label{lem:isotr->tr}
Given a isotrivial family $\calC \to \calB$ of smooth projective irreducible curves, there exists a cover $\calB' \to \calB$ such that the base changed family $\calC \times_\calB \calB' \to \calB'$ is a generically trivial family, i.e. is birational to a product $\calC \times_\C \calB_0$.
\end{lemma}

Lemma \ref{lem:isotr->tr} implies that rational points for curves defined over function fields will not be finite for isotrivial curves. The analogous form of Mordell Conjecture for function fields thus asks whether this holds only for this class of curves. We can then restate Theorem \ref{thm:faltings} in the following way:

\begin{theorem}\label{thm:geo_mordell}
Let $\calC$ be a smooth projective curve defined over a function field $F$ of genus $g(\calC)>1$. If $\calC(F)$ is infinite then $\calC$ is isotrivial.
\end{theorem}

Theorem \ref{thm:geo_mordell} was proved in the sixties by Manin \cite{Manin1963} (although with a gap fixed by Coleman \cite{Coleman1990}) using analytic arguments, and later by Grauert \cite{Grauert1965} using algebraic methods. Samuel in \cite{Samuel1966} gave a proof in characteristic $p$ using ideas of Grauert. A detailed explanation of Grauert methods can be found in Samuel's survey \cite{SamuelTata}. In Mazur's detailed discussion of Faltings' proof of Mordell Conjecture \cite{Mazur1987}, Mazur stresses the role of Arakelov \cite{Arakelov1971} and Zahrin's \cite{Zarhin1974} results which imply new proofs of the Geometric Mordell Conejcture, using ideas of Parshin: this gives even more importance to the geometric case.

One of the ideas of Grauert's proof, which is central in some of the higher dimensional extensions is the following: suppose $\calC$ is a curve defined over a function field $F$ of a curve $\calB$, corresponding to a fibration $\pi: X \to \calB$. Then one can prove that almost all sections of the fibration, which correspond to rational points, verify a first order differential equation, i.e. almost all sections are tangent to a given horizontal vector field. Formally each section $\sigma: \calB \to X$ can be lifted to the projective bundle $\calB \to \PP(\Omega^1_X) = \Proj(\Sym(\Omega_X^1))$ via the surjective map $\sigma^*\Omega^1_X \to \Omega^1_\calB$. Grauert proves (in a different language) that there exists a section $\phi$ of a suitable line bundle over $\PP(\Omega^1)$ whose zero section contains all but finitely many images of sections. Grauert then concludes that if infinitely many sections exist, given the fact that they satisfy the differential equation given by $\phi = 0$, a splitting is provided for the relative tangent sequence which implies that the family is isotrivial (via the vanishing of the Kodaira-Spencer class).

In particular, Grauert's construction gives first insights towards the theory of jet spaces which occupy a central role in some degeneracy results in the complex analytic setting. In this direction, recent analogues of Theorem \ref{thm:geo_mordell} in higher dimension have been proved by Mourougane \cite{Mourougane} for very general hypersurfaces in the projective space of high enough degree using proper extensions of the ideas briefly described above.


\subsection{Vojta Conjecture for Function Fields}\label{ssec:vojta_ff}
Since function fields possess a theory of heights analogous to the theory over number fields, one can translate Vojta's Main Conejcture \ref{conj:Vojta} to the function field case. The main conjecture implies the following height bound for varieties of log general type type over function fields.

\begin{conjecture}\label{conj:vojta_ff}
Let $(\calX,\calD)$ be a pair over a function field $F = k(B)$ whose generic fiber $(X,D)$ is a pair of log general type. Then, for every $\varepsilon > 0$ there exists a constant $C$ and a proper closed subvariety $Z$ such that for all $P (\in \calX \setminus Z) (\overline{F})$ one has
\begin{equation}
    \label{eq:vojta_ff}
    h_{K_\calX + D}(P) \leq C (\chi(P) + N^{(1)}_D(P)) +O(1)
\end{equation}
where, given a point $P \in \calX(L)$ corresponding to a cover $B_P \to B$ of degree $n$, corresponding to the field extension $L \supset F$, we have that $\chi(P) = \chi(B_P)/n$. Moreover, the truncated counting function $N^{(1)}_D (P)$ is the cardinality of the support of $P^*D$.
\end{conjecture}

Note that for varieties of log general type the height in \eqref{eq:vojta_ff} is associated to a big divisor. In this case, if the set of points of bounded height is Zariski dense then the model is isotrivial.
Moreover, if one considers only points defined over $F$ then the characteristic of the point $P$ reduces to $2(g(B)) - 2$ and one recovers the usual conjecture for $(D,S)$-integral points where $\# S \geq N^{(1)}_D(P)$.

In this latter case one can related Conjecture \ref{conj:vojta_ff} to hyperbolicity using the following result of Demailly.

% will not be the focus of the following parts of this Thesis but rather another related formulation slightly weaker that comes from the following observation made in the holomorphic curves setting. Recall that a complex compact manifold is said to be (Brody) \emph{hyperbolic} if every holomorphic map from $\C$ to the manifold is constant; in the compact case Brody hyperbolicity is equivalent to Kobayashi hyperbolicity, equivalence following from Brody's Lemma (see for details \cite{Brody1978}). In particular, for algebraic manifolds, hyperbolicity would imply that all holomorphic maps from abelian varieties must be constant. Kobayashi \cite{Kobayashi1970} and Lang \cite{Lang1986} made conjectures about the relationship between hyperbolicity and algebraic properties of the manifolds and whether such properties would imply, or being equivalent to, hyperbolicity. One consequence of hyperbolicity for compact manifolds is the following: 

\begin{theorem}[Demailly \cite{Demailly1997}]\label{th:AlgHypDemailly}
Let $X$ be a projective complex variety embedded in some projective space for a choice of a very ample line bundle. Then if the associated manifold is Kobayashi hyperbolic the following holds: there exists a constant $A>0$ such that each irreducible curve $\calC \subset X$ satisfies
\[
\deg \calC \leq A (2 g(\tcal{C}) - 2) = A \chi(\tcal{C}),
\]
where $\tcal{C}$ is the normalization of $\calC$.
\end{theorem}

Following this result, Demailly introduced the following notion.

\begin{definition}\label{def:alghyp}
A smooth projective variety $X$ is \emph{algebraically hyperbolic} if there exists a constant $A$ such that for each irreducible curve $\calC \subset X$	the following holds:
\[
\deg \calC \leq A \chi(\tcal{C}).
\]
\end{definition}

Using strong analogies between hyperbolicity and degeneracy of rational points Lang conjectured that a general type variety should be hyperbolic outside a proper exceptional set and therefore one could also conjecture that the variety should be algebraically hyperbolic outside that set (for more on algebraically hyperbolic varieties we refer to \cite{jav,jav2}). This allows one to rephrase Conjeture \ref{conj:vojta_ff} as follows.

\begin{conjecture}[Lang-Vojta for function fields]\label{conj:alghyp}
Given an affine variety $X$ embedded as $\overline{X} \setminus D$ for a smooth projective variety $\overline{X}$ and a normal crossing divisor $D$, if $X$ is of log general type then there exists a proper subvariety $Exc$ (called the \emph{exceptional set}) such that there exists a bound for the degree of images of non-constant morphisms $\calC \to X$ from affine curves whose image is not entire contained in $Exc$, in terms of the Euler Characteristic of $\calC$.
\end{conjecture}

By the previous remark it is easy to see that Conjecture \ref{conj:vojta_ff} implies Conjecture \ref{conj:alghyp}.


We note that most of the known techniques used for the number field case can be used to prove analogous results in the function field setting. However, due to the presence of tools that are not available over number fields, most notably the presence of derivation, one can obtained stronger results that lead to cases of Conjecture \ref{conj:alghyp} and Conjecture \ref{conj:vojta_ff} in settings that are currently out of reach in the function function field case. We refer to the articles \cite{Voloch,BM,Chen,Wang,PR,CZConic,Mourougane,CZGm,Amos,CaTur} as some examples of results over function fields along these lines.

\begin{remark} For the sake of completion, we discuss briefly how \emph{algebraic hyperbolicity} fits in with our previous discussions on hyperbolicity (see \cite[Example 6.3.24]{lazarsfeld2}.
\begin{itemize}
    \item If $X$ is algebraically hyperbolic, then $X$ contains no rational or elliptic curves.
    \item If $X$ is algebraically hyperbolic then there are no non-constant maps $f: A \to X$ from an abelian variety $A$.
    \item Kobayashi (and thus Brody) hyperbolicity implies algebraic hyperbolicity for projective varieties.
\end{itemize}
Furthermore, a theorem of Kobayashi (see \cite[Theorem 6.3.26]{lazarsfeld2}) states that if $\Omega^1_X$ is ample, then $X$ is algebraically hyperbolic. 
\end{remark}



% Euler Characteristic for affine abstract curves was defined in \ref{def:EulerCh} at page \pageref{def:EulerCh}. We stress that Conjecture \ref{conj:alghyp} is a special case of Conjecture \ref{conj:LV2} because maps $\calC \to X$ from an affine curve with normalization $\tcal{C} \setminus S$ correspond to $(S,D)$-integral points for $X$ as defined over the function field of the curve $\calC$. Now a bound for the degree of their images gives an height bound for such integral points and therefore implies that they cannot be Zariski dense in $X$ unless $X$ is not isotrivial.
% Finally we can now state the conjecture we are going to devote most of this Thesis, namely a weaker version of Conjecture \ref{conj:alghyp}: the conjecture deals with logarithmic general type affine varieties in which there could exists curves with negative Euler characteristic. This implies that in general such varieties will not be algebraically hyperbolic. Nevertheless a slight modification of the bound of Theorem \ref{th:AlgHypDemailly} it is expected to hold.

% \begin{conjecture}\label{conj:LV}
% Given $X, \tilde{X}, D$ as before, if $X$ is of log general type then there exists a constant $A$ such that for each affine curve $\calC$ with normalization $\tcal{C}\setminus S$ for a smooth projective curve $\tcal{C}$, a finite set of points $S \subset \tcal{C}$ and for all non-constant morphisms $\varphi : \calC \to X$, the following holds:
% \[
% \deg \varphi (\tcal{C}) \leq A \max \{ 1, \chi_S(\tcalC) \}.
% \]
% \end{conjecture}

% Conjecture \ref{conj:LV} is slightly weaker than Conjecture \ref{conj:alghyp} because it allows maps from curves of non-negative Euler Characteristic to $X$. However, if images of curves with negative Euler characteristic are all contained in a proper subvariety of $X$, e.g. there exist only finitely many images of such curves in $X$, this implies the conclusion of Conjecture \ref{conj:alghyp}. For the property described in the previous Conjecture, being a weaker version of algebraic hyperbolicity, one can give the following



